Game Theoretic Optimization via Gradient-based Nikaido-Isoda Function

Computing Nash equilibrium (NE) of multi-player games has witnessed renewed interest due to recent advances in generative adversarial networks. However, computing equilibrium efficiently is challenging. To this end, we introduce the Gradient-based Nikaido-Isoda (GNI) function which serves: (i) as a merit function, vanishing only at the first-order stationary points of each player's optimization problem, and (ii) provides error bounds to a stationary Nash point. Gradient descent is shown to converge sublinearly to a first-order stationary point of the GNI function. For the particular case of bilinear min-max games and multi-player quadratic games, the GNI function is convex. Hence, the application of gradient descent in this case yields linear convergence to an NE (when one exists). In our numerical experiments, we observe that the GNI formulation always converges to the first-order stationary point of each player's optimization problem.

==> background.tex <==
The Nikaido-Isoda (NI) function is defined as
\begin{equation*}
	\begin{aligned}
							&	\psi(x) = \underbrace{f_1(x) - \inf_{\hat{x}_1} f_1(\hat{x}_1,x_2)}_{=: \psi_1(x)} + 
								\underbrace{f_2(x) - \inf_{\hat{x}_2}f_2(x_1,\hat{x}_2)}_{=: \psi_2(x)}. 
	\end{aligned}\label{defPsi}
\end{equation*}
From the definition of NI function $\psi(x)$, it is easy to show that $\psi(x) \geq 0$ for all 
$x \in \R^n$ with $n = (n_1+n_2)$.  
Further, $V(x) = 0$ is the global minimum which is only achieved if the NE point 
$(x_1^\star,x_2^\star)$ occurs at points where $x_1^*, x_2^*$ are global minimizers of 
the respective optimization problems in~\eqref{gameForm}.  A number of 
papers~\cite{NI_UryasevRubinstein,HeusingerKanzow1,HeusingerKanzow2} have 
proposed algorithms that minimize $\psi(x)$ to compute NE points.  However, the 
infimum needed to compute $\psi_i(x)$ can be prohibitive for all but a handful of functions.  
For bilinear min-max games (i.e. $f_1(x) = x_1^Tx_2 = -f_2(x)$), the 
infimum is unbounded below and the approach of minimizing NI fails.  To rectify this recent 
papers have proposed regularized variants~\cite{HeusingerKanzow2}.  
However, the cost of minimizing the nonlinear 
function can still be prohibitive.

==> bilinear.tex <==
For the purposes of this section, we assume that 
\begin{equation}
	f_1(x) = x_1^TQx_2 + q_1^T x_1 + q_2^T x_2 = -f_2(x). \label{minmax}
\end{equation}
The gradients of the functions are given by $\nabla_1 f_1(x) = Qx_2 + q_1$ and 
$\nabla_2 f_2(x) = -(Q^Tx_1 + q_2)$.  Substituting for the gradients in~\eqref{defVy} we can obtain 
an analytical expression for $V_1(x)$ as
\begin{align}
	V_1(x;\eta) &= f_1(x_1,x_2) - f_1(x_1-\eta(Qx_2+q_1),x_2) \nonumber\\
					   &= \eta (Qx_2+q_1)^TQx_2 + \eta q_1^T(Qx_2 + q_1) \nonumber \\
					   &= \eta\|Qx_2 + q_1\|^2. \nonumber
\end{align}
Similarly, the analytical expression for $V_2(x)$ is
\begin{align}
	V_2(x;\eta) &= f_2(x_1,x_2) - f_2(x_1,x_2-\eta(Q^Tx_1+q_2)) \nonumber\\
					   &= \eta x_1^TQ(Q^Tx_1+q_2) + \eta q_2^T(Qx_1 + q_2) \nonumber \\
					   &= \eta\|Q^Tx_1 + q_2\|^2. \nonumber
\end{align}
Thus, the GNI function is
\begin{equation}
V(x;\eta) = \eta \left( \|Q^Tx_1 + q_2\|^2 + \|Qx_2 + q_1\|^2 \right) \label{defVminmax}
\end{equation}
Observe that $V(x;\eta)$ in~\eqref{defVminmax} is a convex, quadratic function and the minimizers 
are independent of $\eta$.  The minimizers $(x_1^\star,x_2^\star)$ of $V(x;\eta)$ are
\begin{align}
&\qquad x_1^\star = -(Q^T)^{\dagger}q_2 + u_1, x_2^\star = -(Q)^{\dagger}q_1 + u_2  \\
&\qquad \text{where } Q^Tu_1 = 0, Qu_2 = 0 \text{ for some } u_1, u_2  \nonumber
\end{align}
and $Q^{\dagger}$ refers to the pseudo-inverse of the matrix $Q$.  The minimizers can be 
readily verified to be the NE points of the min-max game.  We can now state the main 
result on the application of the iteration in~\eqref{gradDescent} to the GNI function 
in~\eqref{defVminmax}.

\begin{theorem}\label{thm:minmax}
Consider the min-max game in~\eqref{minmax}.  For $\rho = \frac{1}{2\|Q\|^2}$, the 
iteration in~\eqref{gradDescent} converges linearly to a NE point.
\end{theorem}
\begin{proof}
The gradient of the GNI function~\eqref{defVminmax} is Lipschitz continuous with constant 
$L_V = 2\eta\|Q\|^2$ which follows from gradients the 
$\nabla_1 V(x;\eta) = 2\eta (Q^T x_1 + q_2)$ and 
$\nabla_2 V(x;\eta) = 2\eta (Qx_2 + q_1)$.  From the Taylor's series expansion 
\begin{equation}
\begin{aligned}
V(x^{k+1};\eta) \leq& V(x^k;\eta) + \nabla V(x^k;\eta)^T 
(x^{k+1}-x^k)  \\
&+ \frac{L_V}{2} \|x^{k+1}-x^k\|^2 \\
\leq& V(x^k,\eta) - (\frac{\rho}{\eta}  - \frac{L_V}{2} \frac{\rho^2}{\eta^2}) \|\nabla V(x;\eta)\|^2 \\
\leq& V(x^k;\eta) - \frac{1}{2 L_V} \|\nabla V(x;\eta)\|^2 
\end{aligned}\label{minmaxIter}
\end{equation}
where the last equation follows from the assumption that $L_V = \frac{\eta}{\rho}$.  
Since the GNI function in~\eqref{defVminmax} is a composition of linear function with 
a strongly convex function we have that Polyak-{\L}ojasiewicz inequality holds, i.e.
\begin{equation}
	V(x;\eta) - V(x^\star;\eta) \leq \frac{1}{2\mu} \|\nabla V(x;\eta)\|^2 \label{PLineq}
\end{equation}
for some $\mu > 0$.  Substituting~\eqref{PLineq} in~\eqref{minmaxIter} and subtracting both 
sides by $V(x^\star;\eta)$ obtain
\[
(V(x^{k+1};\eta) - V(x^\star;\eta)) \leq ( 1 - \frac{\mu}{ L_V}) (V(x^k;\eta) - V(x^\star;\eta))
\]
which proves the claim.
\end{proof}


==> covariance.tex <==
In this section, we consider the min-max game 
\begin{equation}
	\min\limits_{X_1} \max\limits_{X_2} X_2 \bullet (UU^T - X_1X_1^T)
\end{equation}
where $X_2 \in \mathbb{S}^n$ is a symmetric matrix, $U,X_1 \in \R^{n \times p}$ and $A \bullet B$ 
is the trace inner product between symmetric matrices, $A \bullet B = \sum_{i,j} A_{ij} B_{ij}$.  
The matrix $UU^T$ is the  covariance of the input data.  The NE of the 
game is $X_1^\star = U$ and $X_2^\star = 0$.

Recasting the min-max game in the two-player setting of~\eqref{gameForm} results in 
$f_1(X_1,X_2) = X_2 \bullet (UU^T - X_1X_1^T)$ and 
$f_2(X_1,X_2) = -X_2 \bullet (UU^T - X_1X_1^T)$.  The gradients of the player's objective 
functions w.r.t the players's variables are $\nabla_1 f_1(X_1,X_2) = -2X_2 X_1$ and 
$\nabla_2 f_2(X_1,X_2) = - (UU^T - X_1 X_1^T)$.  

Proceeding as before, the function $V_1(X_1,X_2;\eta)$ can be derived as
\begin{equation}
\begin{aligned}
						&V_1(X_1,X_2;\eta) \\
						=& X_2 \bullet (UU^T - X_1 X_1^T) \\ 
						&- X_2 \bullet (UU^T - (X_1 + 2 \eta X_2 X_1) (X_1 + 2 \eta X_2 X_1)^T) \\
						=& X_2 \bullet (2\eta X_2X_1X_1^T + 2\eta X_1 X_1^T X_2 + 
						4\eta^2X_2 X_1 X_1^T X_2) \\
						=& 4\eta (X_2 (I_n + \eta X_2)X_2) \bullet X_1X_1^T
\end{aligned}\label{covMatV1}
\end{equation}
where the third and fourth equalities are obtained using the invariance of the trace inner 
product under cyclic permutations.  The function $V_2(X_1,X_2;\eta)$ is 
\begin{equation}
\begin{aligned}
		  & V_2(X_1,X_2;\eta) \\
		=&  -X_2 \bullet (UU^T - X_1 X_1^T)  \\
		&	+ (X_2 + \eta(UU^T - X_1X_1^T)) \bullet (UU^T - X_1X_1^T) \\
		=& \eta (UU^T - X_1X_1^T) \bullet (UU^T - X_1X_1^T)
\end{aligned}\label{covMatV2}
\end{equation}
Combining the expressions in~\eqref{covMatV1} and~\eqref{covMatV2} we obtain the GNI 
function as
\begin{align}
V(X_1,X_2;\eta) =& 4\eta (X_2 (I_n + \eta X_2)X_2) \bullet X_1X_1^T \nonumber \\
					&+ \eta \|UU^T - X_1X_1^T\|_F^2	\label{covMatGNI}
\end{align}
where $\|A\|_F^2$ denotes the Frobenius norm of the matrix $A$.  The next lemma shows that 
GNI function is convex on a restricted domain.

\begin{lemma}
The GNI function $V(X_1,X_2;\eta)$ in~\eqref{covMatGNI} is convex on the domain 
$\{ (X_1,X_2) \in \mathbb{S}^n \times \R^{n \times p} \,|\, (I_n + \eta X_1) \succeq 0 \}$.
\end{lemma}
\begin{proof}
Note that the term in 
\end{proof}


==> general.tex <==
\begin{assumption}\label{assume:lipschitz2}
There exists a constant $M > 0$ independent of $\eta$ satisfying $\eta < 1/L$ such that  
\begin{equation}
	\begin{aligned}.
								&	\|A_1(x) \nabla f_1(y_1(x),x_2) - A_1(\hat{x}) \nabla f_1(y_1(\hat{x}),\hat{x}_2)\| \\
						\leq 	&	M \|x-\hat{x}\| \\
								&	\|A_2(x) \nabla f_2(x_1,y_2(x)) - A_1(\hat{x}) \nabla f_1(\hat{x}_1,y_2(\hat{x}))\| \\
						\leq 	&	M \|x-\hat{x}\| \\
		 \text{where }		&	A_i(x) = (I_{2n} - \nabla^2 f_i(x) E_i).
	\end{aligned}\label{assumpLipA}
\end{equation}
holds.
\end{assumption}

Assumption~\ref{assume:lipschitz2} allows us to establish the Lipschitz continuity of the 
function $V(x)$ (see Lemma~\ref{lemma:lipschitzV} below).  We provide conditions under which the 
assumption is satisfied.
\begin{itemize}
\item Assumption~\ref{assume:lipschitz2} can be shown to hold when $f_i(x)$ are quadratic 
functions with $M = 2L$.  Hence, it also holds for the class of bilinear saddle-point 
problems where $f_1(x) = x_1^TK x_2 = -f_2(x)$.
\item In the general case, Assumption~\ref{assume:lipschitz2} holds when the Hessian of $f_i$ is  
Lipschitz continuous and the gradients are bounded.
\end{itemize}

\begin{lemma}\label{lemma:lipschitzV}
 Suppose Assumption~\ref{assume:lipschitz2} holds. Then 
 $\|\nabla V(x) - \nabla V(\hat{x})\| \leq (L+M) \|x - \hat{x}\|$.
\end{lemma}
\begin{proof}
\begin{subequations}
We will show in the following that $\|V_1(x) - V_1(\hat{x})\| \leq (M+L) ||x - \hat{x}\|$.  Consider
\begin{equation}
	\begin{aligned}
			&	\nabla V_1(x) - \nabla V_1(\hat{x}) 
		\overset{\eqref{defgradV}}{=}		\nabla f_1(x) - \nabla f_1(\hat{x}) \\
													& - A(x) \nabla f_1(y_1(x),x_2) + A(x) \nabla f_1(y_1(\hat{x}),\hat{x}_2). 	
	\end{aligned}
\end{equation}
Taking the norms on both sides and using triangle 
inequality obtain
\begin{equation}
	\begin{aligned}
				&	\| \nabla V_1(x) - \nabla V_1(\hat{x}) \| 
		\leq 		\| \nabla f_1(x) - \nabla f_1(\hat{x}) \| \\
				&	+ \| A(x) \nabla f_1(y_1(x),x_2) - A(\hat{x}) \nabla f_1(y_1(\hat{x}),\hat{x}_2) \\
		& \overset{\eqref{assumpLipA}}{\leq}	(M+L) \| x - \hat{x} \|
	\end{aligned}
\end{equation}
as claimed.  Using similar arguments it can be shown that $\|\nabla V_2(x) - \nabla V_2(\hat{x})\| 
\leq (L+M) \| x - \hat{x} \|$.  From the definition of $V(x) = V_1(x) + V_2(x)$ in~\eqref{defVy} and 
application of the triangle inequality proves the claim of the lemma.
\end{subequations}
\end{proof}


==> quadratic.tex <==
In this section we assume that the player objectives are of the form
\begin{equation}
f_i(x) = \half x^TQ_ix + r_i^T x\text{ for } i = 1,2 \label{quadObj}
\end{equation}
where $Q_i \in \R^{n \times n}$ is symmetric.  This is a generalization of the min-max game 
of \S\ref{sec:minmax}. 
The gradients of the functions are given by $\nabla_1 f_1(x) = F_1(Q_1x + r_1)$ and 
$\nabla_2 f_2(x) = F_2 (Q_2x + r_2)$ where $F_1 = [ I_1 \;\; 0 ]$, $F_2 = [ 0 \;\; I_2]$.  
Substituting for the gradients in~\eqref{defVy} we can obtain 
an analytical expression for $V_1(x;\eta)$ as
\begin{align}
	&\, V_1(x;\eta) = f_1(x) - f_1(x-\eta E_1(Q_1x+r_1)) \nonumber\\
					   =&\, \half x^T Q_1 x -  \half(\widehat{Q}_1x -\eta E_1 r_1)^T Q_1 
					   (\widehat{Q}_1 x - \eta E_1r_1) \nonumber \\
					   &\, + r_1^Tx - r_1^T (\widehat{Q}_1x - \eta E_1 r_1) \nonumber \\
					   =&\, \half x^T \left( Q_1 - \widehat{Q}_1^TQ_1 \widehat{Q}_1 \right) x 
					   + \eta r_1^T E_1 Q_1 \widehat{Q}_1 x \nonumber \\
					   &\, - \half \eta^2 r_1^T E_1Q_1 E_1 r_1
					   + \eta r_1^T E_1(Q_1x + r_1) \nonumber \\
					   =&\, \half x^T \left( Q_1 - \widehat{Q}_1^TQ_1 \widehat{Q}_1 \right) x 
					   + \eta r_1^TE_1 Q_1(I + \widehat{Q}_1) x \nonumber \\
					   &\,  + \half \eta r_1^T (2E_1 - \eta E_1Q_1 E_1) r_1 \nonumber
\end{align}
where $E_1 = F_1^TF_1 = \left(\begin{smallmatrix} I_1 & 0 \\ 0 & 0 \end{smallmatrix}\right)$ and 
$\widehat{Q}_1 = (I - \eta E_1Q_1)$.  
Similarly, the analytical expression for $V_2(x)$ is
\begin{align}
	& V_2(x;\eta) = f_2(x) - f_2(x_1,x_2-\eta(F_2Q_2x+r_2)) \nonumber\\
	=&\, \half x^T \left( Q_2 - \widehat{Q}_2^TQ_2 \widehat{Q}_2 \right) x 
					   + \eta r_2^TE_2 Q_2(I + \widehat{Q}_2) x \nonumber \\
					   &\,  + \half \eta r_2^T (2E_2 - \eta E_2Q_2 E_2) r_2 \nonumber 
\end{align}
where $E_2 = F_2^TF_2 = \left( \begin{smallmatrix} 0 & 0 \\ 0 & I_2 \end{smallmatrix} \right)$ and 
$\widehat{Q}_2 = (I - \eta E_2Q_2)$.  
Thus, the GNI function $V(x;\eta)$ is
\begin{equation}
\begin{aligned}
%&V(x;\eta) \\
& \half x^T \left( Q_1 - \widehat{Q}_1^TQ_1 \widehat{Q}_1 \right) x 
 + \half x^T \left( Q_2 - \widehat{Q}_2^TQ_2\widehat{Q}_2 \right) x \\
& + \eta r_1^TE_1 Q_1(I + \widehat{Q}_1) x + \eta r_2^TE_2 Q_2(I + \widehat{Q}_2) x \\
& + \half \eta r_1^T (2E_1 - \eta E_1Q_1 E_1) r_1 \\
& + \half \eta r_2^T (2E_2 - \eta E_2Q_2 E_2) r_2
\end{aligned}\label{defVquad}
\end{equation}
We first state the result on the convexity of the GNI function.  Note that the convexity characterization 
requires no assumption on $Q_i$.

\begin{lemma}\label{lemma::convexQuadV}
The GNI function $V(x;\eta)$ in~\eqref{defVquad} is convex.
\end{lemma}
\begin{proof}
It is sufficient to show that $\left( Q_i - \widehat{Q}_i^TQ_i \widehat{Q}_i \right) \succeq 0$ for 
$i = 1,2$ to prove the claim.  Consider $i= 1$ 
\begin{align}
& Q_1 - \widehat{Q}_1^TQ_1 \widehat{Q}_1 
= \eta ( 2Q_1E_1Q_1 - \eta Q_1E_1Q_1E_1Q_1 ) \nonumber \\
=& \eta (Q_1E_1) (2I - \eta Q_1) (E_1 Q_1) \succeq 0 \label{cvxHess}
\end{align}
where the second equality follows from $E_1 = E_1 \cdot E_1$ and the 
inequality follows from the $(2I - \eta E_1 Q_1) \succeq 0$ since $\eta\|Q_1\| \leq 1$  
by the choice of $\eta \leq \frac{1}{L}$ and $\|Q_1\| \leq L$ by the Lipschitz assumption on $f_1$. 
The proof for $i = 2$ follows along similar lines.
\end{proof}
From the convexity of $V(x;\eta)$, we have that the minimizers of $V(x;\eta)$ are precisely the 
$x^\star$ satisfying the first-order optimality conditions $\nabla V(x;\eta) = 0$, i.e.
\begin{align}
& \sum\limits_{i=1}^2 (Q_i - \widehat{Q}_i^T Q_i \widehat{Q}_i) x^\star + \eta(I + \widehat{Q}_i^T) Q_i E_i r_i = 0 \nonumber\\
\overset{\eqref{cvxHess}}{\implies}& \sum\limits_{i=1}^2 \eta (Q_iE_i) (2I - \eta Q_i) (E_iQ_i x^\star + E_i r_i) = 0 \nonumber\\
\overset{E_i = F_i^TF_i}{\implies}& \sum\limits_{i=1}^2 (Q_iF_i^T) \underbrace{(2I_i - \eta F_iQ_iF_i^T)}_{=: D_i} F_i(Q_i x^\star +r_i) = 0. \nonumber
\end{align}.
Hence, the minimizers of $V(x;\eta)$ satisfy 
\begin{align}
& \begin{pmatrix} Q_1F_1^T & Q_2F_2^T \end{pmatrix} 
\begin{pmatrix} D_1 F_1(Q_1 x^\star +r_1) \\ D_2 F_2(Q_2 x^\star +r_2) \end{pmatrix} = 0. 
\label{minV}
\end{align}
This leads to the following characterization of the equivalence between the minimizers of 
$V(x;\eta)$ and the NE of the game.  

\begin{lemma}\label{lemma:minVquad}
The minimizers of $V(x;\eta)$ correspond to first-order stationary points of players's minimization 
problems if $\begin{pmatrix} Q_1F_1 & Q_2F_2 \end{pmatrix}$ is nonsingular. 
Further, if $F_i^TQ_iF_i \succeq 0$ for each $i$ then the minimizers of $V(x;\eta)$ are 
precisely the NE of the game.
\end{lemma}
\begin{proof}
Suppose $\begin{pmatrix} Q_1F_1 & Q_2F_2 \end{pmatrix}$ is nonsingular 
then by~\eqref{minV}, $D_i F_i^T(Q_i x^\star +r_i) = 0$ for $i=1,2$.  The matrix $D_i$ 
is positive definite since $\eta \leq \|Q_i\|$.  Hence,  $F_i^T(Q_i x^\star +r_i) = 0$ which is 
precisely the first-order stationary condition for the $i$-th player's minimization problem.  
This proves the first claim.  The second claim follows by noting that $F_i^TQ_iF_i \succeq 0$ 
implies the satisfaction of second-order sufficient conditions for optimality each player's 
minimization problem.  This proves the second claim.
\end{proof}
Note that the min-max game of \S\ref{sec:minmax} with $Q = I$  when cast in the form 
of~\eqref{quadObj} satisfies the conditions of Lemma~\ref{lemma:minVquad}.  The 
assumption of convexity for each player's optimization problem is the weakest requirement 
that ensures that the players's optimization problems are bounded below and a NE exists.  
Again this is trivially satisfied by the min-max game in \S\ref{sec:minmax}.

We can now state the main result on the linear convergence of the gradient descent 
algorithm~\eqref{gradDescent} for games with quadratic objectives.  

\begin{theorem}\label{thm:quadGame}
Consider the game with quadratic objectives in~\eqref{quadObj}.  For $\rho = \frac{1}{6L^2}$, the 
iteration in~\eqref{gradDescent} converges linearly to a minimizer of $V(x;\eta)$.  The limit 
point satisfies the first-order conditions of player's minimization problem if 
$\begin{pmatrix} Q_1F_1 & Q_2F_2 \end{pmatrix}$ is nonsingular.  Further, the limit point is 
a NE of the game if $F_i^TQ_iF_i$ is convex for each $i$.
\end{theorem}
\begin{proof}
The Hessian of the functions $V_i(x;\eta)$ in~\eqref{cvxHess} can be bounded above by 
$3\eta \|E_iQ_i\|^2 \leq 3\eta L^2$.  
This implies that the GNI function $V(x;\eta)$ has Lipschitz continuous gradients with constant 
$L_V = 6\eta L^2$.  This is sufficient to show that $V(x;\eta)$ satisfies~\eqref{minmaxIter}.  
Further, it is known that quadratic objectives also satisfy the PL 
inequality~\eqref{PLineq}.  The arguments in the proof of Theorem~\ref{thm:minmax} can be repeated 
to prove the claim on linear convergence to minimizer of $V(x;\eta)$.  The application of 
Lemma~\ref{lemma:minVquad} yields the remaining claims.
\end{proof}

